A/B testing under Interference with Partial Network Information

A/B tests are often required to be conducted on subjects that might have social connections. For e.g., experiments on social media, or medical and social interventions to control the spread of an epidemic. In such settings, the SUTVA assumption for randomized-controlled trials is violated due to network interference, or spill-over effects, as treatments to group A can potentially also affect the control group B. When the underlying social network is known exactly, prior works have demonstrated how to conduct A/B tests adequately to estimate the global average treatment effect (GATE). However, in practice, it is often impossible to obtain knowledge about the exact underlying network. In this paper, we present UNITE: a novel estimator that relax this assumption and can identify GATE while only relying on knowledge of the superset of neighbors for any subject in the graph. Through theoretical analysis and extensive experiments, we show that the proposed approach performs better in comparison to standard estimators.

==> aistats_header <==
% Get better typography
% \usepackage[protrusion=true,expansion=true]{microtype}		

% Small margins
%\usepackage[top=2cm, bottom=2cm, left = 1cm, right = 1cm,columnsep=20pt]{geometry}

\usepackage{theoremref}

% For basic math, align, fonts, etc.
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{bbm}
\usepackage{mathtools}
\usepackage{mathrsfs}
\usepackage{dsfont}
% \usepackage[scr=esstix,cal=boondox]{mathalfa} 

\usepackage{courier} % For \texttt{foo} to put foo in Courier (for code / variables)

\usepackage{lipsum} % For dummy text

% for underlining text

\def\mul#1#2{\color{#1}\underline{{\color{black}#2}}\color{black}}
% \usepackage{soul} 
% \newcommand{\myul}[2][black]{\setulcolor{#1}\ul{#2}\setulcolor{black}}

% For images
% \usepackage{graphicx}
% \usepackage{subcaption}
\usepackage[space]{grffile} % For spaces in image names
\usepackage{cancel} % For diagonally striking out equations
\usepackage{tablefootnote}

% For bibliography
\usepackage{natbib}

% For links (e.g., clicking a reference takes you to the phy)
\usepackage{hyperref}

% For color
\usepackage{graphicx}
\usepackage{wrapfig}
\usepackage{xcolor}
\definecolor{dark-red}{rgb}{0.4,0.15,0.15}
\definecolor{dark-blue}{rgb}{0,0,0.7}
\hypersetup{
    colorlinks, linkcolor={dark-blue},
    citecolor={dark-blue}, urlcolor={dark-blue}
}


% Macros
\newcommand{\yash}[1]{\textcolor{blue}{[#1---yash]}}
\newcommand{\imp}[1]{\textcolor{red}{[IMP: #1]}}
\newcommand{\red}[1]{\textcolor{purple}{[#1]}}

\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}



\usepackage{algpseudocode}
% \usepackage[noend,linesnumbered,ruled]{algorithm2e}
\usepackage[vlined,linesnumbered,ruled,algo2e]{algorithm2e}
% \usepackage[algo2e]{algorithm2e} 
\SetKwProg{Fn}{Function}{}{}
\let\oldnl\nl% Store \nl in \oldnl
\newcommand{\nonl}{\renewcommand{\nl}{\let\nl\oldnl}}% Remove line number for one line


% Miscelaneous headers
\usepackage{multicol}
\usepackage{enumitem}
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{bm}

\newcommand{\ind}{\perp\!\!\!\!\perp}

% Commands for organizing theorems and proofs

\usepackage{theoremref}
\mathtoolsset{showonlyrefs}

\newtheorem{defn}{Definition}[]
\newtheorem{rem}{Remark}[]
\newtheorem{thm}{Theorem}[]
\newtheorem{claim}{Claim}[]
\newtheorem{lemma}{Lemma}[]
\newtheorem{prop}{Property}[]
\newtheorem{ass}{Assumption}[]
\newtheorem{cor}{Corollary}[]

% For creating sub-groups of Assumptions/Theorems etc.
\newtheorem{reqm}{Requirement}
% \renewcommand\thereqm{A\arabic{reqm}}

\usepackage{thmtools}
\usepackage{thm-restate}

\declaretheorem[name=Theorem]{rtheorem}
\declaretheorem[name=Proposition]{rproposition}
\declaretheorem[name=Assumption]{rassumption}
\declaretheorem[name=Corollary]{rcorollary}
\declaretheorem[name=Lemma]{rlemma}


% Definitions of handy macros can go here
\newcommand{\dataset}{{\cal D}}
\newcommand{\fracpartial}[2]{\frac{\partial #1}{\partial  #2}}
\newcommand{\pibopt}{\pi_{b^\star}}
\newcommand{\pib}{{\pi_b}}
\newcommand{\pitheta}{{\pi_\btheta}}
\newcommand{\deltheta}{{\frac{\partial}{\partial \btheta}}}
\newcommand{\delthetatwo}{{\frac{\partial^2}{\partial^2 \btheta}}}
\newcommand{\pieval}{{\pi_e}}
\newcommand{\btheta}{{\boldsymbol\theta}}
\newcommand{\data}{{\mathcal{D}}}
\newcommand{\ope}{{\operatorname{OPE}}}
\newcommand{\pe}{{\operatorname{PE}}}
\newcommand{\variance}{{\operatorname{Var}}}
\newcommand{\covariance}{{\operatorname{Cov}}}
\newcommand{\bias}{{\operatorname{Bias}}}
\newcommand{\mse}{{\operatorname{MSE}}}
\newcommand{\loss}{{\mathcal{L}}}
\newcommand{\horizon}{{l}}

% Auto sized brackets
\DeclarePairedDelimiter\autobracket{(}{)}
\newcommand{\br}[1]{\autobracket*{#1}}

\DeclarePairedDelimiter\autobrackett{[}{]}
\newcommand{\brr}[1]{\autobrackett*{#1}}

\DeclarePairedDelimiter\autobrackettt{\{}{\}}
\newcommand{\brrr}[1]{\autobrackettt*{#1}}
